Universal Backdoor Attacks Detection via Adaptive Adversarial Probe

Extensive evidence has demonstrated that deep neural networks (DNNs) are vulnerable to backdoor attacks, which motivates the development of backdoor attacks detection. Most detection methods are designed to verify whether a model is infected with presumed types of backdoor attacks, yet the adversary is likely to generate diverse backdoor attacks in practice that are unforeseen to defenders, which challenge current detection strategies. In this paper, we focus on this more challenging scenario and propose a universal backdoor attacks detection method named Adaptive Adversarial Probe (A2P). Specifically, we posit that the challenge of universal backdoor attacks detection lies in the fact that different backdoor attacks often exhibit diverse characteristics in trigger patterns (i.e., sizes and transparencies). Therefore, our A2P adopts a global-to-local probing framework, which adversarially probes images with adaptive regions/budgets to fit various backdoor triggers of different sizes/transparencies. Regarding the probing region, we propose the attention-guided region generation strategy that generates region proposals with different sizes/locations based on the attention of the target model, since trigger regions often manifest higher model activation. Considering the attack budget, we introduce the box-to-sparsity scheduling that iteratively increases the perturbation budget from box to sparse constraint, so that we could better activate different latent backdoors with different transparencies. Extensive experiments on multiple datasets (CIFAR-10, GTSRB, Tiny-ImageNet) demonstrate that our method outperforms state-of-the-art baselines by large margins (+12%).

==> resources/temp.tex <==
\iffalse
\begin{figure}[htb]
	\centering
	\begin{minipage}{0.15\linewidth}
		\centering
		
		\centerline{\includegraphics[width=\textwidth]{CVPR 2023/latex/pic/bad-s.png}}
		\centerline{(a)}
% 		\caption{}
% 		\label{fig:trigger_size}
	\end{minipage}
	%\qquad
	\begin{minipage}{0.15\linewidth}
		\centering
		\centerline{\includegraphics[width=\textwidth]{CVPR 2023/latex/pic/bad-l.png}}
		\centerline{(b)}
% 		\caption{}
% 		\label{fig:trigger_transparency}%文中引用该图片代号
	\end{minipage}
	%\qquad
	\begin{minipage}{0.15\linewidth}
		\centering
		\centerline{\includegraphics[width=\textwidth]{CVPR 2023/latex/pic/blend-h.png}}
		\centerline{(c)}
% 		\caption{}
% 		\label{fig:trigger_transparency}%文中引用该图片代号
	\end{minipage}
	%\qquad
	\begin{minipage}{0.15\linewidth}
		\centering
		\centerline{\includegraphics[width=\textwidth]{CVPR 2023/latex/pic/blend-l.png}}
		\centerline{(d)}
% 		\caption{}
% 		\label{fig:trigger_transparency}%文中引用该图片代号
	\end{minipage}
	%\qquad
	\begin{minipage}{0.15\linewidth}
		\centering
		\centerline{\includegraphics[width=\textwidth]{CVPR 2023/latex/pic/wanet.png}}
		\centerline{(e)}
% 		\caption{}
% 		\label{fig:trigger_transparency}%文中引用该图片代号
	\end{minipage}
	%\qquad
	\begin{minipage}{0.15\linewidth}
		\centering
		\centerline{\includegraphics[width=\textwidth]{CVPR 2023/latex/pic/input-aware.png}}
		\centerline{(f)}
% 		\caption{}
% 		\label{fig:trigger_transparency}%文中引用该图片代号
	\end{minipage}
	
	\caption{Visualization of backdoor attacks used in our experiments. (a)-(b) BadNets with different trigger sizes; (c)-(d) Blend with different trigger transparencies; (e) WaNet; (f) Input-Aware.}
	\label{fig:tot_trigger}
\end{figure}

\fi

==> src/temp.tex <==
\subsection{Box-to-Sparsity Budget Scheduling} 

After finding the optimal region, the next step is to inject adversarial probes into the image. However, as challenge \ding{183} indicated, different trigger transparencies also impact the detection performance. Thus, a question emerges: \emph{can we modify the attack budget to an arbitrary value?}

To explore the problem, we conduct adversarial attacks on the whole image region with different attack budgets (as shown in Fig \ref{fig:budget confusion matrix}). On one hand, with a proper attack budget, the output of infected models would skew to the target label, while the clean models show no obvious deviation; on the other hand, if the attack budget is increased to an extremely large value (\eg, 32/255), the model output would collapse due to the excessive attack. \emph{Therefore, we should find a suitable budget within the specific region}, which satisfies (1) the adversarial probe could successfully activate the latent backdoor and (2) the budget value does not damage model predictions. Thus, we introduce the box-to-sparsity constraints budget scheduling strategy.

% Generally, it is necessary to maintain the strength of the adversarial attack within a certain range, based on which we propose a box-constrained budget scheduling.

% The box-constrained budget scheduling is a strategy that adaptively adjusts budget for adversarial probe as region decreasing to guarantee L2 of probe distributes stably within a certain range. In other words, probe will gradually become sparse.
% whether an image is over-attacked. For example, when ASR-A is 1, the image is likely to be over-attacked.
For clarity, we use the Attack Success Rate of an adversarial attack (\ie, ASR-A) to measure the attack strength. At the initial stage $t_0$, our attacking region $\bm{r}^{(0)}$ is the whole image, and the attacks at this stage should be treated as box-constrained perturbations. Specifically, we first pre-define a threshold $\xi$ that controls the extent to activate the backdoor trigger, \ie, ASR-A $\in$ $[\xi,1)$. The reason is that a too-low ASR-A value implies a small number of adversarial examples for outlier detector, which will be insufficient for backdoor detection. Then, we implement a binary search to find the optimal attack budget at stage 0, which suffices to achieve high ASR-A satisfying $\xi$. Considering that the excessive attack would jeopardize backdoor activation, we set ASR-A $\omega$ at stage 0 as the attacking boundary to limit the subsequent budget scheduling process.
%Specifically, while scheduling the attack budget, the ASR-A in the following stages should be smaller than the initial stage to prevent an excessive attack, which may mislead a clean model as an infected one. Since it is time-consuming to search for an optimal budget at each stage, for simplicity, we maintain the $\ell_{2}$-norm of perturbation within a certain range to ensure the total value of perturbation stable.

%Existing backdoor detections, usually using the adversarial attack with box-constraints (i.e., $\ell_{\infty}$, $\ell_{1}$, $\ell_{2}$) to activate the latent backdoor. 
As the region shrinks in the subsequent stages, we should incrementally improve the attacking budget that achieves comparatively high ASR-A that is close to $\omega$. Thus, the budget for stage $t$ should be formulated as
\begin{equation}
    \bm{\delta}^{(t)} = \bm{\delta}^{(t-1)} + \kappa(\epsilon_{\mathcal{\delta}}),
\end{equation}
where $\kappa(\cdot)$ is a function that finds the optimal increment for budget at stage $t$ based on step size $\epsilon_{\mathcal{\delta}}$. Specifically, we first keep adding $\bm{\delta}^{(t-1)}$ by $\epsilon_{\mathcal{\delta}}$ until find a budget leading to excessive attack; we then follow by a binary search strategy to calculate the actual budget for stage $t$. To decrease the time consumption, we set the biggest increment as $3 \times \epsilon_{\mathcal{\delta}}$. 

As the stage continues, we iteratively increase the attack budget while reducing the perturbing region without limitation on the values of the adversarial attack. From this point of view, at this time, our attack area becomes sparser, and our adversarial perturbations are scheduled from the box constraint (\eg, $\ell_2$) to the sparse constraint ($\ell_{0}$). In sum, we adjust the attack budget via the box-to-sparsity scheduling which simulate different trigger patterns to ensure the diversity of hidden backdoor activation (see Section \ref{sec:abs} for discussions).




%At the initial stage, we utilize a global region and a small budget, which could be considered as the box-constrained attack. Specifically, for each stage, we inject adversarial perturbation on each sample $\bm{x}_{i}$ through several attack iterations as
%\begin{equation}
%\bm{\delta}_{j} = \varepsilon * sign(\nabla_{\bm{x}_{i}^{j} \odot \bm{r}_{i}^{(t)}} \mathcal{L}(f_{\theta}(\bm{x}_{i}^{j}), \bm{y}_{i})),
%\end{equation}
%where $\beta$ is the step size and $\bm{x}_{i}^{j}$ is the intermediate adversarial example at iteration $j$. We then clip the pixel values exceeding the attack budget $\mathcal{B}^{t}$ as
%\begin{equation}
%\bm{x}_{i}^{j} = \bm{x}_{i}^{j-1} \odot (1 - \bm{r}_{i}^{(t)}) + \Pi_{\mathcal{B}^{(t)}}( \bm{\delta}_{j-1} \odot \bm{r}_{i}^{(t)}).
%\end{equation}

% As the area shrinks and the budget increases, our attack area becomes sparser. Therefore, the adversarial perturbations would be scheduled from the box constraint (\eg, $\ell_{\infty}$) to the sparse constraint ($\ell_{0}$). Next, we do not stop increasing the budget but continue to increase the attack budget while reducing the perturbed area, i.e., not limiting the values of the adversarial attack. At this time, the adversarial attack is converted to an attack under the sparse constraint. In conclusion, we schedule the budget via the box to sparsity constraints schedule, which generates adversarial perturbations (probes) from box-constrained adversarial attack to sparsity adversarial attack.




% To design the schedule from the box constraint (\eg, $\ell_{\infty}$) to the sparse constraint ($\ell_{0}$), . to-sparsity budget scheduling 
% As the area shrinks and the budget increases, our attack area becomes sparser, which motivates us to design the box-to-sparsity budget scheduling. 
% (1) For the region at each stage, we set 





% \textbf{Box to Sparsity constraints} Rethinking our region shrinking strategy, which transits from global region to sparse mask, our objective also turns from adversarial attack constrained by $\ell_{\infty}$-norm to $\ell_{0}$-norm attack with attention to certain pixels. At the initial stage, we utilize a global region and a small budget, which could be considered as the box-constrained adversarial attack (i.e., $\ell_{\infty}$, $\ell_{1}$, $\ell_{2}$). As the region shrinks and the budget increases, our attack becomes more and more sparse and high-intensity pixel-wise, similar to the sparsity adversarial attack. In conclusion, we increase the budget via box-constrained to sparsity budget schedule, which generates adversarial perturbations (probes) from box-constrained adversarial attack to sparsity adversarial attack. We demonstrate that our multi-stage detection method could simulate multiple backdoor triggers due to various probe generation methods. Notably, to our knowledge, a sparsity adversarial attack is not mentioned in the field of backdoor detection because it is non-convex.


% Interestingly, we also notice that the ASR-a shows a decreasing trend without sacrificing backdoor detection accuracy. Such phenomenon indicates that those samples which could be attacked by both box-constrained attack and sparse attack are critical for backdoor detection. 
% while sparsity adversarial attack  At the initial stage, with global region and small budget, the attack strategy is equivalent to $\ell_{\infty}$-norm attack, which xxx. As region shrinking and budget increasing, our attack strategy gradually turns to $\ell_{0}$-norm attack. Therefore, we 
